Single Pulse Detection Algorithms for Real-time Fast Radio Burst Searches using GPUs

The detection of non-repeating or irregular events in time-domain radio astronomy has gained importance over the last decade due to the discovery of fast radio bursts. Existing or upcoming radio telescopes are gathering more and more data and consequently the software, which is an important part of these telescopes, must process large data volumes at high data rates. Data has to be searched through to detect new and interesting events, often in real-time. These requirements necessitate new and fast algorithms which must process data quickly and accurately. In this work we present new algorithms for single pulse detection using boxcar filters. We have quantified the signal loss introduced by single pulse detection algorithms which use boxcar filters and based on these results, we have designed two distinct "lossy" algorithms. Our lossy algorithms use an incomplete set of boxcar filters to accelerate detection at the expense of a small reduction in detected signal power. We present formulae for signal loss, descriptions of our algorithms and their parallel implementation on NVIDIA GPUs using CUDA. We also present tests of correctness, tests on artificial data and the performance achieved. Our implementation can process SKA-MID-like data 266$\times$ faster than real-time on a NVIDIA P100 GPU and 500x faster than real-time on a NVIDIA Titan V GPU with a mean signal power loss of 7%. We conclude with prospects for single pulse detection for beyond SKA era, nanosecond time resolution radio astronomy.

==> hardware.tex <==
\begin{table*}[!ht]
	\caption{\label{tab:hardware}GPU card specifications. The shared memory bandwidth is calculated as $\mathrm{BW (bytes/s)} = \mathrm{(bank\, bandwidth\, (bytes))} \times \mathrm{(clock\, frequency\, (Hz))} \times \mathrm{(32\, banks)} \times \mathrm{(\#\, multiprocessors)}$.}
	\centering
	\begin{tabular}{|l|r|r|}
	\hline
	\textbf{} & \textbf{P100} & \textbf{TITAN V} \\
	\hline
	Total CUDA Cores & 3584 & 5120 \\
	%\hline
	Streaming Multiprocessors (SMs) & 56 & 80 \\
	%\hline
	Base/Max Core Clock & 1126/1303 MHz & 1220/1455 MHz \\
	%\hline
	Memory Clock & 1406 MHz & 850 MHz \\
	%\hline
	Global memory bandwidth & 720 GB/s & 652 GB/s \\
	%\hline
	Shared memory bandwidth & 9121 GB/s & 14550 GB/s \\
	%\hline
	Global memory size & 16 GB & 12 GB\\
	%\hline
	TDP & 250 W & 250 W\\
	%\hline
	CUDA version & 8.0.44 & 9.1.85\\
	%\hline
	Driver version & 384.81 & 387.34\\
	\hline
	\end{tabular}
\end{table*}
